Lower Complexity Bounds of Finite-Sum Optimization Problems: The Results and Construction

In this paper, we study the lower complexity bounds for finite-sum optimization problems, where the objective is the average of $n$ individual component functions. We consider Proximal Incremental First-order (PIFO) algorithms which have access to the gradient and proximal oracles for each component function. To incorporate loopless methods, we also allow PIFO algorithms to obtain the full gradient infrequently. We develop a novel approach to constructing the hard instances, which partitions the tridiagonal matrix of classical examples into $n$ groups. This construction is friendly to the analysis of PIFO algorithms. Based on this construction, we establish the lower complexity bounds for finite-sum minimax optimization problems when the objective is convex-concave or nonconvex-strongly-concave and the class of component functions is $L$-average smooth. Most of these bounds are nearly matched by existing upper bounds up to log factors. We can also derive similar lower bounds for finite-sum minimization problems as previous work under both smoothness and average smoothness assumptions. Our lower bounds imply that proximal oracles for smooth functions are not much more powerful than gradient oracles.

==> minimax/average.tex <==
\subsection{Construction for the Average Smooth Case}
\label{sec:minimax:average}
In this subsection, we consider the lower bounds of PIFO complexity under the the average smooth assumption.

\subsubsection{Strongly-Convex-Strongly-Concave Case}
We first consider the minimax problem where the objective function is strongly-convex in $\vx$ and strongly-concave in $\vy$.

Without loss of generality, we assume $\mu_x \ge \mu_y$. 
For fixed $L', \mu_x, \mu_y, R_x, R_y, n, \eps$ such that  $L / \mu_x \ge 2$, we set $L = \sqrt{\frac{n(L'^2 - 2 \mu_x^2 )}{2} + 2 \mu_x^2}$, and consider $\{f_{\text{SCSC}, i}\}_{i=1}^n$ and $f_{\text{SCSC}}$ defined in Definition \ref{defn:scsc}.
Let $\kappa_x' = L / \mu_x$ and $\kappa_y' = L / \mu_y$. We have the following proposition.
\begin{proposition}\label{prop:average:strongly-strongly:example}
For any $n \ge 4$ and $\kappa'_x = \frac{L'}{\mu_x} \ge 2$, we have that
\begin{enumerate}
    \item $f_{\text{SCSC}}(\vx, \vy)$ is $(\mu_x, \mu_y)$-convex-concave and $\{f_{\text{SCSC}, i}\}_{i=1}^n$ is $L'$-average smooth.
    \item $\frac{\sqrt{n}}{2} L' \le L \le \sqrt{\frac{n}{2}} L'$ and $\kappa_x = \frac{L}{\mu_x} \ge 2$.
\end{enumerate}
\end{proposition}
\begin{proof}
\begin{enumerate}
    \item Clearly, $f_{\text{SCSC}} (\vx, \vy)$ is $(\mu_x, \mu_y)$-convex-concave. 
    % By Corollary \ref{coro:convex-concave:base-scale}, 
    By Proposition \ref{prop:convex-concave:base} and Lemma \ref{lem:scale},
    $\{ f_{\text{SCSC}, i} (\vx, \vy) \}$ is $\hat{L}$-average smooth where
    \begin{align*}
        \hat{L} = \frac{ \sqrt{ L^2 - 2 \mu_x^2 } }{2n} \sqrt{ 8n + \frac{8 n^2}{ L^2 / \mu_x^2 - 2 } }
        = \sqrt{ \frac{ L'^2 - 2 \mu_x^2 }{ 8n} } \sqrt{ 8n + \frac{ 16n }{ L'^2 / \mu_x^2 - 2 }} = L'.
    \end{align*}
    \item It is easy to check the second inequality. For the first inequality, we find that 
    \begin{align*}
        L^2 - \frac{n}{4} L'^2 = \frac{n}{4} L'^2 - (n-2) \mu_x^2
        = \mu_x^2 \left( \frac{n}{4} \kappa_x'^2 - n + 2  \right)
        \ge \mu_x^2 (n - n + 2) \ge 0.
    \end{align*}
    Since $n \ge 4$, we have $\kappa_x = \frac{L}{\mu_x} \ge \frac{ \sqrt{n} L' }{2 \mu_x} \ge 2$.
\end{enumerate}
This completes the proof.
\end{proof}
% \bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L, \mu_x, \mu_y)
% \Omega\left(\left(n {+} \sqrt{ \kappa_x \kappa_y n } \right)\log\left(1/\eps \right)\right), &\text{ for } \kappa_x, \kappa_y = \Omega(\sqrt{n}), \\
% \Omega\left(\left(n {+} n^{3/4} \sqrt{\kappa_y }\right)\log\left(1/\eps \right)\right), &\text{ for } \kappa_y = \Omega(\sqrt{n}), \kappa_x = \fO(\sqrt{n}), \\
% \Omega\left( n \right), &\text{ for } \kappa_x, \kappa_y = \fO(\sqrt{n}),.

Now we give the proof of Theorem \ref{thm:average:strongly-strongly}.

\begin{proof}[Theorem \ref{thm:average:strongly-strongly}]
\begin{enumerate}
    \item For $\kappa_y' \ge \kappa_x' = \Omega(\sqrt{n} )$, consider the minimax problem (\ref{prob:scsc}) where $L = \sqrt{\frac{n(L'^2 - 2 \mu_x^2 )}{2} + 2 \mu_x^2}$. By Theorem \ref{thm:strongly-strongly} and Proposition \ref{prop:average:strongly-strongly:example}, we have \[
    \bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', \mu_x, \mu_y) = \Omega\left(\left(n {+} \sqrt{ \kappa_x' \kappa_y' n } \right)\log\left(1/\eps \right)\right).
    \]
    \item For $\kappa_y' = \Omega(\sqrt{n})$ and $\kappa_x' = \fO(\sqrt{n})$, we set $L = \sqrt{\frac{n(L'^2 - \mu_y^2)}{2} - \mu_y^2}$ and consider $\{ G_{\text{SCSC}, i} \}_{i=1}^n $, $G_{\text{SCSC}}$, $\fX$ and $\fY$ defined in the proof of Theorem \ref{thm:scsc:example:2}. 
    By Proposition \ref{prop:average:strongly:example}, we know that $G_{\text{SCSC}}$ is $(\mu_x, \mu_y)$-convex-concave, $\{ G_{\text{SCSC}, i} \}_{i=1}^n$ is $L'$-average smooth,
    $\frac{ \sqrt{n} }{2} L' \le L \le \sqrt{ \frac{n}{2} } L'$ and $\kappa_y = L / \mu_y \ge 2$.
    Following the proof of Theorem \ref{thm:scsc:example:2}, we can obtain  \[
    \bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', \mu_x, \mu_y) = \Omega\left(\left(n {+} n^{3/4} \sqrt{\kappa_y' }\right)\log\left(1/\eps \right)\right) .\]
    \item For $\kappa_x', \kappa_y' = \fO(\sqrt{n})$, note that $\{ H_{\text{SCSC}, i} \}_{i=1}^n$ defined in Lemma \ref{lem:scsc:example:3} is also $L$-average smooth. Then we have $\bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L, \mu_x, \mu_y) = \Omega\left( n \right) $.
\end{enumerate}
This completes the proof.
\end{proof}

% We first restate Theorem \ref{thm:average:strongly-strongly} as follows.
% \begin{theorem}\label{thm:average:scsc:example}
% For any $L', \mu_x, \mu_y, n, R_x, R_y, \eps$ such that $\mu_x > 0$, $\mu_y > 0$ $\kappa'_x = L' / \mu_x \ge 2$, $\kappa'_y = L' / \mu_y \ge 2$, $n \ge 4$ and $\eps \le  \min \left\{ \frac{ n \mu_x R_x^2}{800 \kappa_x' \kappa_y'}, \frac{\mu_y R_y^2}{1600}, \frac{L'R_x^2}{4} \right\}$,  
% % $\eps \le LR^2/4$,

% \begin{enumerate}
%     \item $n \ge 4$ $\kappa_y' \ge \kappa_x' = \Omega(\sqrt{n} )$. For $\eps \le \min \left\{ \frac{ n \mu_x R_x^2}{800 \kappa_x' \kappa_y'}, \frac{\mu_y R_y^2}{1600} \right\} $
%     there exists a dimension $d = \fO \left( 1 + \sqrt{ \frac{ \kappa_x' \kappa_y'} {n} } \log \left(1/\eps\right) \right) $ and $n$ functions $\{f_i:\BR^d \times \BR^d \rightarrow \BR\}_{i=1}^n$  such that $f(\vx, \vy) \in \bar{\fF}_{\mathrm{CC}}(R_x, R_y, L', \mu_x, \mu_y)$ and $\bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', \mu_x, \mu_y) = \Omega\left(\left(n {+} \sqrt{ \kappa_x' \kappa_y' n } \right)\log\left(1/\eps \right)\right)$.
%     \item $n \ge 4$ $\kappa_y' = \Omega(\sqrt{n})$ $\kappa_x' = \fO(\sqrt{n})$ $\eps \le \frac{1}{720} \mu_y R_y^2$  there exists a dimension $d = \fO \left( 1 + \frac{ \sqrt{ \kappa_y' }}{n^{1/4}} 
%      \log \left(1/\eps\right) \right) $ and $n$ functions $\{f_i:\BR^d \times \BR^d \rightarrow \BR\}_{i=1}^n$  such that $f(\vx, \vy) \in \bar{\fF}_{\mathrm{CC}}(R_x, R_y, L', \mu_x, \mu_y)$ and $\bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', \mu_x, \mu_y) =  \Omega\left(\left(n {+} n^{3/4} \sqrt{\kappa_y' }\right)\log\left(1/\eps \right)\right) $
%     \item $ \kappa_x', \kappa_y' = \fO(\sqrt{n} )$ $\eps \le \frac{L' R_x^2}{4}$ there exist $n$ functions $\{f_i:\BR \times \BR \rightarrow \BR\}_{i=1}^n$  such that $f(\vx, \vy) \in \bar{\fF}_{\mathrm{CC}}(R_x, R_y, L', \mu_x, \mu_y)$ and $\bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', \mu_x, \mu_y) = \Omega(n) $
% \end{enumerate}
% \end{theorem}

% \begin{proof}
% \begin{enumerate}
%     \item Set $L = \sqrt{\frac{n(L'^2 - 2 \mu_x^2 )}{2} + 2 \mu_x^2}$, and consider $\{f_{\text{SCSC}, i}\}_{i=1}^n$, $f_{\text{SCSC}}$ and problem (\ref{prob:scsc}) defined in Definition \ref{defn:scsc}.
    
%     Next, we prove that $\frac{\sqrt{n}}{2} L' \le L \le \sqrt{\frac{n}{2}} L'$.
%     It is easy to check the second inequality. For the first inequality, we find that 
%     \begin{align*}
%         L^2 - \frac{n}{4} L'^2 = \frac{n}{4} L'^2 - (n-2) \mu_x^2
%         = \mu_x^2 \left( \frac{n}{4} \kappa_x'^2 - n + 2  \right)
%         \ge \mu_x^2 (n - n + 2) \ge 0.
%     \end{align*}
%     Since $n \ge 4$, we have $\kappa_x = \frac{L}{\mu_x} \ge \frac{ \sqrt{n} L' }{2 \mu_x} \ge 2$. By Theorem \ref{thm:strongly-strongly}, we obtain the first result of Theorem \ref{thm:average:scsc:example}.
%     \item Set $L = \sqrt{\frac{n(L'^2 - \mu_y^2)}{2} - \mu_y^2}$ and consider $\{ \tilde{g}_i \}_{i=1}^n $, $\tilde{g}$ defined in Theorem \ref{thm:scsc:example:2}. 
%     By Proposition \ref{prop:average:strongly:example}, $\tilde{g}(\vx, \vy)$ is $(\mu_x, \mu_y)$-convex-concave and $\{\tilde{g}_i\}_{i=1}^n$ is $L'$-average smooth. 
%     Moreover, we have $\frac{ \sqrt{n} }{2} L' \le L \le \sqrt{ \frac{n}{2} } L$ and $\kappa_y = L / \mu_y \ge 2$.
%     Following the proof of Theorem \ref{thm:scsc:example:2}, we can obtain the second result of Theorem \ref{thm:average:scsc:example}.
%     \item Note that $\{ \tilde{h}_i \}_{i=1}^n$ defined in Lemma \ref{lem:scsc:example:3} is also $L$-average smooth. The third result follows from Lemma \ref{lem:scsc:example:3}.
% \end{enumerate}
% \end{proof}
% For fixed $L', \mu_x, \mu_y, R_x, R_y, n, \eps$ such that $\mu_x \ge \mu_y$ and $L / \mu_x \ge 2$, we set $L = \sqrt{\frac{n(L'^2 - 2 \mu_x^2 )}{2} + 2 \mu_x^2}$, and consider $\{f_{\text{SCSC}, i}\}_{i=1}^n$, $f_{\text{SCSC}}$ and problem (\ref{prob:scsc}) defined in Definition \ref{defn:scsc}. We have the following proposition.

\subsubsection{Convex-Strongly-Concave Case}
We now consider the minimax problem where the objective function is convex in $\vx$ and strongly-concave in $\vy$.

For fixed $L', \mu_y, R_x, R_y, n, \eps$ such that $L' / \mu_y \ge 2$, we set $L = \sqrt{\frac{n(L'^2 - 2 \mu_x^2 )}{2} + 2 \mu_x^2}$, and consider $\{f_{\text{CSC}, i}\}_{i=1}^n$ and $f_{\text{CSC}}$ defined in Definition \ref{defn:csc}.
Similar to Proposition \ref{prop:average:strongly-strongly:example}, we have the following result.
\begin{proposition}\label{prop:average:convex-strongly:example}
For any $n \ge 4$ and $\kappa'_y = \frac{L'}{\mu_y} \ge 2$, we have that
\begin{enumerate}
    \item $f_{\text{CSC}}(\vx, \vy)$ is $(0, \mu_y)$-convex-concave and $\{f_{\text{CSC}, i}\}_{i=1}^n$ is $L'$-average smooth.
    \item $\frac{\sqrt{n}}{2} L' \le L \le \sqrt{\frac{n}{2}} L'$ and $\kappa_y = \frac{L}{\mu_y} \ge 2$.
\end{enumerate}
\end{proposition}

Then we give the proof of Theorem \ref{thm:average:convex-strongly}.

\begin{proof}[Theorem \ref{thm:average:convex-strongly}]
Consider the minimax problem (\ref{prob:csc}).
By Theorem \ref{thm:csc:example} and Proposition \ref{prop:average:convex-strongly:example}, for $\eps \le \min \left\{ \frac{L'^2 R_x^2}{10368\, n \mu_y}, \frac{\mu_y R_y^2}{36} \right\}$, we have 
\[
    \mathfrak{m}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', 0, \mu_y)=
    \Omega\left(n {+}
    R_x L' \sqrt{ \frac{n}{\mu_y \eps} } \right).
\]
Moreover, consider $\{ G_{\text{CSC}, i} \}_{i=1}^n $, $ G_{\text{CSC}} $, $\fX$ and $\fY$ defined in the proof Theorem \ref{thm:csc:example:2} with $L = \sqrt{\frac{n(L'^2 - \mu_x^2)}{2} - \mu_x^2}$. By Theorem \ref{thm:csc:example:2} and Proposition \ref{prop:average:strongly:example}, for $\eps \le \frac{R_x^2 L'}{768 \sqrt{n} }$,
we have
\[
    \mathfrak{m}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', 0, \mu_y)=
    \Omega\left(n {+} R_x n^{3/4} \sqrt{ \frac{L'}{\eps} }  \right).
\]
Note that $ \{ H_{\text{SCSC}, i} \}_{i=1}^n$ defined in the proof of Lemma \ref{lem:scsc:example:3} is also $L$-average smooth. Then for $\eps \le L' R_x^2 / 4$, we can get the lower bound $\Omega(n)$. Since $\eps \ge \frac{L'^2 R_x^2}{10368\, n \mu_y} $ implies $\Omega (n) = \Omega\left(n {+} R_x L' \sqrt{ \frac{n}{\mu_y \eps} } \right)$ and $\eps \ge \frac{R_x^2 L'}{768 \sqrt{n} }$ implies that $\Omega (n) = \Omega\left(n {+} R_x n^{3/4} \sqrt{ \frac{L'}{\eps} }  \right)$, we obtain that
for $\eps \le \min \left\{ \frac{L' R_x^2}{4}, \frac{\mu_y R_y^2}{36} \right\}$, $\bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', 0, \mu_y)= \Omega\left(n {+} R_x n^{3/4}\! \sqrt{ \frac{L'}{\eps} }  {+} R_x L' \sqrt{ \frac{n}{\mu_y \eps} } \right)$.

Finally, consider $\{ H_{\text{CSC}, i}\}_{i=1}^n$ and $H_{\text{CSC}}$ defined in the proof of Theorem \ref{thm:convex-strongly}, where $g_{\text{SC}} $ is $\mu_y$-convex and $\{ g_{\text{SC}, i}\}_{i=1}^n$ is $L'$-average smooth.
By Theorem \ref{thm:average:strongly}, for $\eps \le L' R_y^2 / 4$ and $L' / \mu_y = \Omega(\sqrt{n})$, we have $\bar{\mathfrak{m}}_{\eps}^{\mathrm{CC}}(R_x, R_y, L', 0, \mu_y)=  n^{3/4}\! \sqrt{\frac{L'}{\mu_y} } \log \left( \frac{1}{\eps} \right)$. This completes the proof.
\end{proof}

\subsubsection{Convex-Concave Case}
For the general convex-concave case,  
% For fixed $L', R_x, R_y, n, \eps$, 
we set $L = \sqrt{\frac{n}{2}}L'$, and consider $\{f_{\text{CC}, i}\}_{i=1}^n$, $f_{\text{CC}}$ and Problem (\ref{prob:cc}) defined in Definition \ref{defn:cc}.
By Proposition \ref{prop:convex-concave:base} and Lemma \ref{lem:scale},
% \ref{coro:convex-concave:base-scale}, 
$\{f_{\text{CC}, i}\}_{i=1}^n$ is $L'$-average smooth.
Then Theorem \ref{thm:cc:example} implies that for $\eps \le \frac{L' R_x R_y}{72 \sqrt{n}}$, the lower bound is $\Omega \left( n + \frac{ \sqrt{n} L' R_x R_y}{\eps} \right)$.

Note that $\{ H_{\text{CC}, i} \}_{i=1}^n $ defined in the proof of Lemma \ref{lem:cc:example:2} is also $L$-average smooth. Then for $\eps \le L' R_x R_y / 4$, we get the lower bound $\Omega(n)$. Since $\eps \ge \frac{L' R_x R_y}{72 \sqrt{n}}$ implies that $ \Omega(n) = \Omega \left( n + \frac{ \sqrt{n} L' R_x R_y}{\eps} \right)$, we obtain the lower bound $\Omega \left( n + \frac{ \sqrt{n} L' R_x R_y}{\eps} \right)$ when $\eps \le L' R_x R_y / 4$.

Following the proof of Theorem \ref{thm:convex-strongly}, for $\eps \le L' R_x^2 / 4$, we can also get the lower bound $\Omega\left(n {+} R_x n^{3/4} \sqrt{ \frac{L'}{\eps} }  \right)$. Similarly, for $\eps \le L' R_y^2 / 4$, we get the lower bound $\Omega\left(n {+} R_y n^{3/4} \sqrt{ \frac{L'}{\eps} }  \right)$. 

In summary, we obtain the result of Theorem \ref{thm:average:convex-concave}.
% By Theorem \ref{thm:convex-concave} and \ref{thm:average:convex-strongly}, we have Theorem \ref{thm:average:convex-concave}.

\subsubsection{Nonconvex-Strongly-Concave Case}
The analysis for the nonconvex-strongly-concave case under the average smooth assumption is similar to that under the smooth assumption. It is based on the following construction.
\begin{definition}\label{defn:average:ncsc}
For fixed $L', \mu_x, \mu_y, \Delta, n$, we define $\bar{f}_{\text{NCSC}, i}: \BR^{m+1} \times \BR^{m+1}  \rightarrow \BR$ as follows
\begin{align*}
    \bar{f}_{\text{NC}, i}(\vx, \vy) = \lambda \hat{r}_i\left(\vx / \beta, \vy / \beta; 
    m + 1,
    \sqrt[4]{\alpha}, \hat{\vc} \right), \text{ for } 1 \le i \le n,
\end{align*}
where
\begin{align*}
    \alpha & = \min \left\{1, \frac{32n \mu_y}{135 L'}, \frac{128 (\sqrt{3} + 1) n \mu_x \mu_y}{45 L'^2} \right\}, \;
    \hat{\vc} = \left( \frac{16 \sqrt{n} \mu_y}{L'}, \frac{\sqrt{\alpha} L' }{16 \sqrt{n} \mu_y }, \sqrt[4]{\alpha}  \right) ,\; \\
    \lambda & = \frac{5308416 n^{3/2} \mu_y^2 \eps^2}{L'^3 \alpha},\;
    \beta = 4 \sqrt{\lambda \sqrt{n} / L'}
    \; \mbox{ and } \; 
    m = \floor{\frac{\Delta L'^2 \sqrt{\alpha}}{3483648 n \eps^2 \mu_y}}.
\end{align*}
Consider the minimiax problem
\begin{equation}
    \min_{\vx \in \BR^{m+1}}\max_{\vy \in \BR^{m+1}} \bar{f}_{\text{NCSC}}(\vx, \vy) \triangleq \frac{1}{n}\sum_{i=1}^n \bar{f}_{\text{NCSC},i}(\vx, \vy). \label{prob:average:ncsc}
\end{equation}
Define $\bar{\phi}_{\text{NCSC}} (\vx) = \max_{\vy \in \BR^{m+1}} \bar{f}_{\text{NCSC}} (\vx, \vy)$.
\end{definition}

Then we have the following proposition.

\begin{proposition}\label{prop:average:nonconvex-strongly}
For any $n \ge 2$, $L' / \mu_y \ge 4$ and $\eps^2 \le \frac{\Delta L'^2 \alpha}{6967296 n \mu_y}$,the following properties hold:
\begin{enumerate}
    \item $\bar{f}_{\text{NCSC}, i}$ is $ (- \mu_x, \mu_y)$-convex-concave and $\{ \bar{f}_{\text{NCSC}, i} \}_{i=1}^n$ is $L'$-average smooth. 
    \item $\bar{\phi}_{\text{NCSC}}(\vzero_{m+1}) - \min_{\vx \in \BR^{m+1}} \bar{\phi}_{\text{NCSC}}(\vx^*) \le \Delta$.
    \item $m \ge 2$ and for $M = m-1$, $\min_{\vx \in \fF_{M}} \norm{\nabla \bar{\phi}_{\text{NCSC}}(\vx)} \ge  9 \eps.$
\end{enumerate}
\end{proposition}
The proof of Proposition \ref{prop:average:nonconvex-strongly} is given in Appendix Section \ref{appendix:minimax}.

Now we give the proof of Theorem \ref{thm:average:nonconvex-strongly}.
\begin{proof}[Theorem \ref{thm:average:nonconvex-strongly}]
By Proposition \ref{prop:nonconvex-strongly}, $f_{\text{NCSC}} (\vx, \vy ) \in \bar{\fF}_{NCC} (\Delta, L' ,\mu_x, \mu_y)$.
% Following from Lemma \ref{lem:minimiax:base} with $H(\vx, \vy) = \norm{\nabla \bar{\phi}_{\text{NCSC} } (\vx)}$, 
Combining Lemma \ref{lem:minimax:ncsc:base} and the third property of Proposition \ref{prop:average:nonconvex-strongly},
for $N = n m / 4$, we have
\[
\min_{t \le N} \E \norm{ \nabla \bar{\phi}_{\text{NCSC} } (\vx_t) } \ge \eps.
\]
Thus, in order to find $(\hat{\vx}, \hat{\vy})$ such that $\E \norm{\nabla \bar{\phi}_{\text{NCSC} } (\hat{\vx})} < \eps$, $\fA$ needs at least $N$ PIFO queries, where
\begin{align*}
    N = \frac{nm}{4} = \Omega \left( \frac{\Delta L'^2 \sqrt{\alpha} }{ \eps^2 \mu_y} \right).
\end{align*}
Since $\eps^2 \le \frac{\Delta L'^2 \alpha}{6967296 n \mu_y}$ and $\alpha \le 1$, we have $\Omega \left( \frac{\Delta L'^2 \sqrt{\alpha} }{ \eps^2 \mu_y} \right) = \Omega \left( n +  \frac{\Delta L'^2 \sqrt{\alpha} }{ \eps^2 \mu_y} \right)$.
\end{proof}



==> minimax/strongly-strongly_old.tex <==
% \subsection{Construction for the Smooth Case}\label{sec:minimax:smooth}
\subsection{Construction for the Strongly-Convex-Strongly-Concave Case}\label{sec:minimax:scsc}
We first consider the finite-sum minimax problem where the objective function is strongly-convex in $\vx$ and strongly-concave in $\vy$.
% each individual component is strongly-convex-strongly-concave.

Without loss of generality, we assume $\mu_x \ge \mu_y$. Denote $\kappa_x = L / \mu_x$ and $\kappa_y = L / \mu_y$. Then we have $\kappa_y \ge \kappa_x$.
The construction can be divided into three parts referred to Sections \ref{sec:minimax:scsc:case1}, \ref{sec:minimax:scsc:case2} and \ref{sec:minimax:scsc:case3}.

\subsubsection{\texorpdfstring{$\kappa_x, \kappa_y = \Omega(n)$}{Case 1}
% {Both the condition numbers are at least linear in n } 
}
\label{sec:minimax:scsc:case1}
For the case $\kappa_x, \kappa_y = \Omega(n)$, the analysis depends on the following construction.

\begin{definition}\label{defn:scsc}
For fixed $L, \mu_x, \mu_y, R_x, R_y$ and $n$ such that $\mu_x \ge \mu_y$, $\kappa_x = L / \mu_x \ge 2$ and $\kappa_y = L / \mu_y \ge 2$,
% denote $\kappa_x = L / \mu_x$, $\kappa_y = L / \mu_y$ and $\alpha = \sqrt{ \frac{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y  }{ n^2 } + 1}$.
we define $f_{\text{SCSC}, i} : \BR^m \times \BR^m \rightarrow \BR$ as follows
\begin{align*}
    f_{\text{SCSC}, i} (\vx, \vy) = \lambda \tilde{r}_i\left(\vx/\beta, \vy/\beta; m, \sqrt{\frac{2}{\alpha + 1}}, \tilde{\vc} \right), \text{ for } 1 \le i \le n,
\end{align*}
where 
\begin{align*}
    \alpha & = \sqrt{ \frac{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y  }{ n^2 } + 1}, \quad
    \tilde{\vc}  = \left( \frac{ 2n }{ \sqrt{\kappa_x^2 - 2} },\, \frac{ 2 n \kappa_x }{ \kappa_y \sqrt{\kappa_x^2 - 2} } \right), \\
    \beta & = \min \left\{ 
    2 n R_x \sqrt{ \frac{\alpha }{ \kappa_x^2 - 2  }}
    ,\, 
    \frac{ 2 n R_x }{ \alpha + 1 } \sqrt{ \frac{ 2 \alpha }{ \kappa_x^2 - 2 } }
    ,\,
    \frac{ \sqrt{ 2 \alpha} R_y  }{ \alpha - 1 }
    % ,\,
    % \frac{  4 n^2 \sqrt{\alpha} R_y }{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y }
    \right\} \text{  and  }
    \lambda  = \frac{ \beta^2 }{ 2n } \sqrt{ L^2 - 2 \mu_x^2 }.
\end{align*}
Consider the minimax problem 
\begin{align}
    \min_{\vx \in \fX}\max_{\vy \in \fY} f_{\text{SCSC}}(\vx, \vy) \triangleq \frac{1}{n}\sum_{i=1}^n f_{\text{SCSC},i}(\vx, \vy). \label{prob:scsc}\\[-0.8cm]\nonumber
\end{align}
where $\fX = \{ \vx \in \BR^m : \norm{\vx} \le R_x  \}$ and
$\fY = \{ \vy \in \BR^m : \norm{\vy} \le R_y  \}$.
Define $\phi_{ \text{SCSC} } (\vx) = \max_{\vy \in \fY} f_{\text{SCSC}} (\vx, \vy)$ and
$\psi_{ \text{SCSC} } (\vy) = \min_{\vx \in \fX} f_{\text{SCSC}} (\vx, \vy) $.
\end{definition}
Then we have the following proposition.
\begin{proposition}\label{prop:strongly-strongly}
For any $n \ge 2$, $m \ge 2$, $f_{\text{SCSC}, i}$ and $f_{\text{SCSC}}$ in Definition \ref{defn:scsc} satisfy:
\begin{enumerate}
    \item $f_{\text{SCSC}, i}$ is $L$-smooth and $(\mu_x, \mu_y)$-convex-concave. Thus, $f_{\text{SCSC}}$ is $(\mu_x, \mu_y)$-convex-concave.
    \item The saddle point of Problem (\ref{prob:scsc}) is
        \begin{align*}
            \begin{cases}
            \vx^* = \frac{ 2 n \beta \mu_y }{ (1-q) \sqrt{L^2 - 2 \mu_x^2} }   (q, q^{2}, \dots, q^m)^{\top}, \\[0.15cm]
            \vy^* = \beta \left(q, q^2, \dots, q^{m-1}, \sqrt{\frac{\alpha+1}{2}} q^m\right)^{\top},
            \end{cases}
        \end{align*}
        where $q=\frac{\alpha-1}{\alpha+1}$.
    %Moreover, $F_{\text{SC}}(\vx^*) = -\Delta$. \label{scp2}
    Moreover, $\norm{\vx^*} \le R_x$, $\norm{\vy^*} \le R_y$.
    % $\Delta = \frac{\beta^2 \xi^2}{ 2 \mu_x}$
    \item For $1 \le k \le m - 1$, we have
    \begin{align*}
    \min_{\vx \in \fX \cap \fF_k} \phi_{\text{SCSC}} (\vx) -
    \max_{\vy \in \fY \cap \fF_k} \psi_{\text{SCSC}} (\vy) \ge  
    % \min_{\vx \in \fF_k} \phi_{\text{SCSC}} (\vx) -
    % \max_{\vy \in \fF_k} \psi_{\text{SCSC}} (\vy) \ge 
    \frac{ \beta^2 \left( L^2 - 2 \mu_x^2 \right) }{ 4 n^2 (\alpha + 1) \mu_x } q^{2k}.
    \end{align*}
\end{enumerate}
\end{proposition}
The proof of Proposition \ref{prop:strongly-strongly} is given in Appendix Section \ref{appendix:minimax}.

We can now prove the lower bound complexity for finding % $\fO(\eps)$-saddle point 
$\eps$-suboptimal point
of Problem (\ref{prob:scsc}) by PIFO algorithms.

\begin{theorem}\label{thm:scsc:example}
Consider the minimax problem (\ref{prob:scsc}) and $\eps>0$.
Let $\kappa_x = L / \mu_x$, $\kappa_y = L / \mu_y$
and $\alpha = \sqrt{ \frac{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y  }{ n^2 } + 1}$.
Suppose that 
\begin{align*}
    & n \ge 2, \, \kappa_y \ge \kappa_x \ge \sqrt{n^2 + 2},\ 
    \eps \le \frac{1}{1600} \min \left\{ \frac{ n^2 \mu_x R_x^2}{ \kappa_x \kappa_y}, \mu_y R_y^2 \right\} , \\
    & \text{and } 
    m = \left\lfloor \frac{\alpha}{4}\log \left(\frac{ \max  \left\{ \mu_x R_x^2, \mu_y R_y^2 \right\} }{9\eps}\right) \right\rfloor + 1.
\end{align*}
In order to find $(\hat{\vx}, \hat{\vy}) \in \fX \times \fY$ such that $ \E \phi_{\text{SCSC}} (\hat{\vx}) - \E \psi_{\text{SCSC}} (\hat{\vy}) < \eps$, PIFO algorithm $\fA$ needs at least $N$ queries, where
% $f_{\text{SCSC}}(\vx, \vy) \in \fF_{\mathrm{CC}}(R_x, R_y, L, \mu_x, \mu_y)$ and 
\begin{align*}
    N =
    \Omega\left(\left(n + \sqrt{\kappa_x \kappa_y}\right)\log\left( \frac{1}{\eps} \right)\right).
\end{align*}
\end{theorem}

\begin{proof}
Let $q = \frac{\alpha - 1}{\alpha + 1}$. 
% We use the same definition of $q$ as Lemma \ref{lem:ssp:sc}.
For $\kappa_y \ge \kappa_x \ge \sqrt{n^2 + 2}$, we have
$\alpha = \sqrt{ \frac{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y  }{ n^2 } + 1} \ge \sqrt{2}$, 
$q = \frac{\alpha - 1}{\alpha + 1} \ge \frac{\sqrt{2} - 1}{\sqrt{2} + 1}$ and $\kappa_x - 2 / \kappa_x \ge \kappa_x / 2$.

Denoting $M = \floor{\frac{ \log \left( 9 (\alpha + 1) \mu_x \eps / \beta^2 \xi^2 \right) }{2\log q}}$ where $\xi = \frac{\sqrt{L^2 - 2 \mu_x^2}}{2n}$, we have
\[
\min_{\vx \in \fX \cap \fF_M} \phi_{\text{SCSC}} (\vx)
- \max_{\vy \in \fY \cap \fF_M} \psi_{\text{SCSC}} (\vy)
% \min_{\vx \in \fF_M} \phi_{\text{SCSC}} (\vx)
% - \max_{\vy \in \fF_M} \psi_{\text{SCSC}} (\vy)
\ge \frac{\beta^2 \xi^2}{(\alpha+1) \mu_x } q^{2M}
\ge 9 \eps.
\]
where the first inequality follows from the third property of Proposition \ref{prop:strongly-strongly}.

First, we need to ensure $1 \le M < m$.
Note that $M \ge 1$ is equivalent to $\eps \le \frac{q^2 \beta^2 \xi^2}{9 (\alpha + 1) \mu_x}$.
% Now we give an upper and lower bound of $\frac{ 9 (\alpha + 1) \mu_x }{ \beta^2 \xi^2}$.
Recall that 
\[
\beta = \min \left\{ 
2 n R_x \sqrt{ \frac{\alpha }{ \kappa_x^2 - 2  }}
,\, 
\frac{ 2 n R_x }{ \alpha + 1 } \sqrt{ \frac{ 2 \alpha }{ \kappa_x^2 - 2 } }
,\,
\frac{ \sqrt{ 2 \alpha} R_y  }{ \alpha - 1 }
% ,\,
% \frac{  4 n^2 \sqrt{\alpha} R_y }{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y }
\right\}  .
\]
When $\beta = 2 n R_x \sqrt{ \frac{\alpha }{ \kappa_x^2 - 2  }}$,
we have
\[
\frac{q^2 \beta^2 \xi^2}{9 (\alpha + 1) \mu_x}
=\frac{ \alpha (\alpha - 1)^2 }{9 (\alpha + 1)^3} \mu_x R_x^2
\ge \frac{\sqrt{2} \left( \sqrt{2} - 1 \right)^5 }{9} \mu_x R_x^2.
\]
When $\beta = \frac{ 2 n R_x }{ \alpha + 1 } \sqrt{ \frac{ 2 \alpha }{ \kappa_x^2 - 2 } }$, recalling that $\alpha^2 - 1 = \frac{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y }{n^2} \le \frac{\kappa_x \kappa_y}{n^2}$,  we have
\[
\frac{q^2 \beta^2 \xi^2}{9 (\alpha + 1) \mu_x}
= \frac{2 \alpha (\alpha - 1)^3 }{ 9 (\alpha + 1)^5 (\alpha-1)} \mu_x R_x^2
\ge \frac{2 \sqrt{2} \left( \sqrt{2} - 1 \right)^7}{9} \frac{n^2 \mu_x R_x^2}{\kappa_x \kappa_y}. 
\]
When $\beta = \frac{ \sqrt{ 2 \alpha} R_y  }{ \alpha - 1 }$, recalling that $\frac{\mu_x \mu_y}{\xi^2} = \frac{4}{\alpha^2 - 1}$, we have
\[
\frac{q^2 \beta^2 \xi^2}{9 (\alpha + 1) \mu_x}
= \frac{ \alpha (\alpha - 1) }{18 (\alpha+1)^2 } \mu_y R_y^2
\ge \frac{\sqrt{2} \left( \sqrt{2} - 1 \right)^3 }{18}  \mu_y R_y^2.
\]
Thus, $\eps \le \frac{1}{1600} \min\left\{ \frac{n^2 \mu_x R_x^2}{\kappa_x \kappa_y}, \mu_y R_y^2 \right\}$ is a sufficient condition for $M \ge 1$.
On the other hand, we have
\begin{align*}
\frac{q^2 \beta^2 \xi^2}{9 (\alpha + 1) \mu_x \eps}
& \le \min \left\{ 
\frac{ \alpha (\alpha - 1)^2 }{9 (\alpha + 1)^3} \mu_x R_x^2,
\frac{2 \alpha (\alpha - 1)^3 }{ 9 (\alpha + 1)^5 (\alpha-1)} \mu_x R_x^2,
\frac{ \alpha (\alpha - 1) }{18 (\alpha+1)^2 } \mu_y R_y^2
\right\} \\
& \le \frac{1}{9} \min \{ \mu_x R_x^2, \mu_y R_y^2 \}.
\end{align*}
Note that the function $h(\beta) = \frac{1}{\log \left(\frac{\beta + 1}{\beta - 1}\right)} - \frac{\beta}{2}$ is increasing when $\beta>1$ and $\lim_{\beta \rightarrow +\infty} h(\beta) = 0$. Thus there holds
\begin{align*}
    \frac{\alpha}{2} + h(\sqrt{2}) \le -\frac{1}{\log q} \le \frac{\alpha}{2}.
\end{align*}
Then we have
\[
m 
= \left\lfloor \frac{\alpha}{4}\log \left(\frac{ \max  \left\{ \mu_x R_x^2, \mu_y R_y^2 \right\} }{9\eps}\right) \right\rfloor + 1
\ge \left\lfloor - \frac{ \log \left(\frac{q^2 \beta^2 \xi^2}{9 (\alpha + 1) \mu_x \eps}\right) }{2 \log q}  \right\rfloor + 1
> M.
\]

% Following from
By Lemma \ref{lem:minimiax:base}, for $M \ge 1$ and $N = (M + 1)n/4$, we have
\[
\min_{t \le N}  \E \phi_{\text{SCSC}} (\vx_t) - \min_{t \le N} \E \psi_{\text{SCSC}} (\vy_t) \ge \eps.
\]
Therefore, in order to find $(\hat{\vx}, \hat{\vy}) \in \fX \times \fY$ such that $\E \phi_{\text{SCSC}} (\hat{\vx}) - \E \psi_{\text{SCSC}} (\hat{\vy}) \ge \eps$,  $\fA$ needs at least $N$ PIFO queries.


At last, we can estimate $N$ by 
{\small\begin{align*}
    -\frac{1}{\log(q)} &= \frac{1}{\log \left(\frac{\alpha + 1}{\alpha - 1}\right)} 
    \ge \frac{\alpha}{2} + h \left( \sqrt{2} \right) \\
    & = \frac{1}{2}\sqrt{\frac{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y }{n^2} + 1} + h \left( \sqrt{2} \right) \\
    & \ge \frac{1}{2}\sqrt{\frac{\kappa_x \kappa_y }{2n^2} + 1} + h \left( \sqrt{2} \right) \\
    & \ge \frac{\sqrt{2}}{4} \left( \sqrt{ \frac{ \kappa_x \kappa_y }{2 n^2} } + 1 \right) + h \left( \sqrt{2} \right) \\
    &\ge \frac{ \sqrt{\kappa_x \kappa_y } }{4n}  + \frac{\sqrt{2}}{4} + h \left( \sqrt{2} \right),
\end{align*}}
and 
{\small\begin{align*}
    N &= (M+1) n/4 \\
    %= \frac{n}{2} \floor{\frac{\log (18\eps)}{2\log q}} \\
    &\ge \frac{n}{4} \left( -\frac{1}{\log(q)} \right) \log \left( \frac{ \beta^2 \xi^2 }{ 9 (\alpha + 1) \mu_x \eps } \right) \\
    &\ge \frac{n}{4}\left( \frac{ \sqrt{\kappa_x \kappa_y } }{4n} + \frac{\sqrt{2}}{4} + h \left( \sqrt{2} \right)  \right) \log \left( \frac{ \min \left\{ n^2 \mu_x R_x^2 / \kappa_x \kappa_y, \mu_y R_y^2 \right\} }{ 1600 \eps }  \right) \\
    &= \Omega\left( \left( n + \sqrt{\kappa_x \kappa_y} \right) \log\left( \frac{1}{\eps} \right) \right).
\end{align*}}
This completes the proof.
\end{proof}

%We emphasize that our lower bound in Theorem \ref{thm:ssp:scsc} also holds under a weaker assumption that $f$ is $(\mu, \mu)$-convex-concave in problem (\ref{prob:main}) and each individual component $f_i$ is only $(0,0)$-convex-concave. 
%We emphasize that our lower bound in Theorem \ref{thm:ssp:scsc} also holds with a weaker assumption that each individual component $f_i$ is convex-concave and $f$ is $(\mu, \mu)$-convex-concave in problem (\ref{prob:main}).



\subsubsection{ \texorpdfstring{ $\kappa_x = \fO(n)$, $\kappa_y = \Omega(n)$}{Case 2}
% {One of the condition numbers is at least linear in n, the other is at most linear in n} 
} \label{sec:minimax:scsc:case2}
For the case $\kappa_x = \fO(n)$, $\kappa_y = \Omega(n)$, we have the following result.
\begin{theorem}\label{thm:scsc:example:2}
% Consider minimax problem (\ref{prob:scsc}) and $\eps>0$ such that
For any $L, \mu_x, \mu_y, n, R_x, R_y, \eps$ such that
\begin{align*}
    & n \ge 2, \, \kappa_y  \ge \sqrt{n^2 + 2} \ge \kappa_x \ge 2,\ 
    \eps \le \frac{1}{720} \mu_y R_y^2 , \\ 
    & \text{and } 
    m = \left\lfloor \frac{1}{4} \left( \sqrt{ \frac{ 2(\kappa_y-1) }{n} + 1 } \right) \log \left(\frac{\mu_y R_y^2  }{9\eps}\right) \right\rfloor + 1,
\end{align*}
where $\kappa_x = L / \mu_x$ and $\kappa_y = L / \mu_y$,
% and $\alpha = \sqrt{ \frac{ \left( \kappa_x - 2 / \kappa_x \right) \kappa_y  }{ n^2 } + 1}$,
there exist n functions $\{ f_i : \BR^m \times \BR^m \rightarrow \BR \}_{i=1}^n$ such that $f_i(\vx, \vy)$ is $L$-smooth and $f(\vx, \vy) = \frac{1}{n} \sum_{i=1}^n f_i(\vx, \vy)$ is $(\mu_x, \mu_y)$-convex-concave. 
Let $\fX = \{ \vx \in \BR^m : \norm{\vx} \le R_x  \}$ and
$\fY = \{ \vy \in \BR^m : \norm{\vy} \le R_y  \}$. 
In order to find $(\hat{\vx}, \hat{\vy}) \in \fX \times \fY$ such that $ \E \max_{\vy \in \fY} f (\hat{\vx}, \vy) - \E \min_{\vx \in \fX} f (\vx ,\hat{\vy}) < \eps$, PIFO algorithm $\fA$ needs at least $N$ queries, where
% $f(\vx, \vy) \in \fF_{\mathrm{CC}}(R_x, R_y, L, \mu_x, \mu_y)$ and
\begin{align*}
    N =
    \Omega\left(\left(n + \sqrt{n \kappa_y}\right)\log\left( \frac{1}{\eps} \right)\right).
\end{align*}
\end{theorem}


\begin{proof}
Let $\alpha = \sqrt{ \frac{ 2 (\kappa_y - 1) }{n} + 1 }$.
Consider the functions $\{ f_{\text{SC}, i} \}_{i=1}^n$ and $f_{\text{SC}}$ defined in Definition \ref{defn:sc} with $\mu$ and $R$ replaced by $\mu_y$ and $R_y$.
% Recall the class of function defined in Section \ref{sec:min:frame} and
We construct  $ \{ G_{\text{SCSC}, i} \}_{i=1}^n, G_{\text{SCSC}}: \BR^m \times \BR^m \rightarrow \BR $ as follows
\begin{align*}
    % g_i (\vx, \vy) & = \frac{\mu_x}{2} \norm{\vx}^2  - f_{i} \left( \vy; m, 0, \sqrt{\frac{2}{\alpha+1}}, \frac{2n}{\kappa_y - 1}, 0, 1, \frac{2 \mu_y R_y^2 \alpha n}{\kappa_y - 1}, \frac{2 R_y \sqrt{\alpha} n }{\kappa_y - 1}  \right) \\
    G_{\text{SCSC}, i} (\vx, \vy) & = \frac{\mu_x}{2} \norm{\vx}^2 - f_{\text{SC},i}(\vy), \\
    % g (\vx, \vy) & = \frac{1}{n} g_i (\vx, \vy) = \frac{\mu_x}{2} \norm{\vx}^2  - \frac{L-\mu_y}{4n} \norm{\mB\left(m, 0, \sqrt{\frac{2}{\alpha + 1}}\right) \vy}^2 - \frac{\mu_y}{2} \norm{\vy}^2  - \mu R_y \sqrt{\alpha} \inner{\ve_1}{\vy}.
    G_{\text{SCSC}} (\vx, \vy) & =  \frac{1}{n} \sum_{i=1}^n G_{\text{SCSC}, i} (\vx, \vy) = \frac{\mu_x}{2} \norm{\vx}^2  - f_{\text{SC}}(\vy).
\end{align*}
By Proposition \ref{prop:base} and Lemma \ref{lem:scale}, 
% \ref{coro:base-scale},
we can check that each component function $G_{\text{SCSC}, i}$ is $L$-smooth and $(\mu_x, \mu_y)$-convex-concave. 
Then $G_{\text{SCSC}}$ is $(\mu_x, \mu_y)$-convex-concave. 
Moreover, we have
\[
% \phi(\vx) = 
\max_{\vy \in \fY} G_{\text{SCSC}}(\vx, \vy) = \frac{\mu_x}{2} \norm{\vx}^2 - \min_{\vy \in \fY} f_{\text{SC}} (\vy)
\quad \text{and} \quad
% \psi(\vy) = 
\min_{\vx \in \fX} G_{\text{SCSC}}(\vx, \vy) = f_{\text{SC}}(\vy).
\]
It follows that for any $(\hat{\vx}, \hat{\vy}) \in \fX \times \fY$, we have
\[
% \phi(\vx) - \psi(\vy) 
\max_{\vy \in \fY} G_{\text{SCSC}}(\hat{\vx}, \vy) - \min_{\vx \in \fX} G_{\text{SCSC}}(\vx, \hat{\vy})
\ge f_{\text{SC}}(\hat{\vy}) -  \min_{\vy \in \fY} f_{\text{SC}} (\vy).
\]
%$\phi(\vx) = \max_{\vy \in \fY} g(\vx, \vy) = \frac{\mu_x}{2} \norm{\vx}^2 - \min_{\vy \in \fY} f_{SC} (\vy)$,
%$\psi(\vy) = \min_{\vx \in \fX} f(\vx, \vy) = f_{SC}(\vy)$
%and $\phi(\vx) - \psi(\vy) \ge f_{SC}(\vy) -  \min_{\vy \in \fY} f_{SC} (\vy) $.
Note that $\kappa_y \ge \sqrt{n^2 + 2 } \ge n/2 + 1$.
By Theorem \ref{thm:strongly:example},
for 
\[
    \eps \le \frac{\mu_y R_y^2}{18} \left(\frac{\alpha-1}{\alpha+1}\right)^{2} \text{ and } 
    m = \left\lfloor \frac{1}{4}\left(\sqrt{\frac{ 2 (\kappa_y - 1) }{n} + 1}\right) \log \left(\frac{\mu_y R_y^2}{9\eps}\right) \right\rfloor + 1,
\]
% $\tilde{g}(\vx, \vy) \in \fF_{\mathrm{CC}}(R_x, R_y, L, \mu_x, \mu_y)$
% and $\mathfrak{m}_{\eps}^{\mathrm{CC}}(R_x, R_y, L, \mu_x, \mu_y)=     \Omega\left(\left(n + \sqrt{n \kappa_y}\right)\log\left( \frac{1}{\eps} \right)\right)$. 
% Therefore, 
in order to find $(\hat{\vx}, \hat{\vy}) \in \fX \times \fY$ such that $\E\left( \max_{\vy \in \fY} G_{\text{SCSC}}(\hat \vx, \vy) - \min_{\vx \in \fX} G_{\text{SCSC}}(\vx, \hat \vy) \right) < \eps$, PIFO algorithm $\fA$ needs at least $N = \Omega\left(\left(n + \sqrt{n \kappa_y}\right)\log\left( \frac{1}{\eps} \right)\right)$ queries.

% From the results in Section \ref{sec:min:smooth:strongly},
% in order to find $(\vx, \vy) \in \fX \times \fY$ such that $\E \phi (\vx) - \E \psi (\vy) \ge \eps$,  $\fA$ needs at least $N$ PIFO queries with $N = \Omega \left( n + \sqrt{n \kappa_y} \log \left( \frac{1}{\eps} \right) \right) $
Moreover, $\kappa_y \ge n/2 + 1$ implies $\alpha \ge \sqrt{2}$. Then we have
$ \left(\frac{\alpha-1}{\alpha+1}\right)^{2} \ge \left( \frac{\sqrt{2} - 1}{\sqrt{2} + 1} \right)^2 \ge \frac{1}{40}$. This completes the proof.
\end{proof}

\subsubsection{ \texorpdfstring{ $\kappa_x, \kappa_y = \fO(n)$}{Case 3}
% {Both the condition number are at most linear in n}
}
\label{sec:minimax:scsc:case3}

For the case $\kappa_x, \kappa_y = \fO(n)$, we can apply the following lemma.
\begin{lemma}\label{lem:scsc:example:3}
% Consider minimax problem (\ref{prob:scsc}) and $\eps>0$ such that
For any $L, \mu_x, \mu_y, n, R_x, R_y, \eps$ such that $n \ge 2$, $L \ge \mu_x$, $L \ge \mu_y$ and $\eps \le \frac{1}{4} L R_x^2$,
there exist n functions $\{ f_i : \BR \times \BR \rightarrow \BR \}_{i=1}^n$ such that $f_i(x, y)$ is $L$-smooth and $f(x, y) = \frac{1}{n} \sum_{i=1}^n f_i(x, y)$ is $(\mu_x, \mu_y)$-convex-concave. 
Let $\fX = \{ x \in \BR : |x| \le R_x  \}$ and
$\fY = \{ y \in \BR : |y| \le R_y  \}$. 
In order to find $(\hat{x}, \hat{y}) \in \fX \times \fY$ such that $ \E \max_{y \in \fY} f (\hat{x}, y) - \E \min_{x \in \fX} f (x ,\hat{y}) < \eps$, PIFO algorithm $\fA$ needs at least $N = \Omega(n)$ queries.
% $f(\vx, \vy) \in \fF_{\mathrm{CC}}(R_x, R_y, L, \mu_x, \mu_y)$ and
% \begin{align*}
%     \mathfrak{m}_{\eps}^{\mathrm{CC}}(R_x, R_y, L, \mu_x, \mu_y) =
%     %\Omega\left(\left(n + \sqrt{n \kappa_y}\right)\log\left( \frac{1}{\eps} \right)\right)
%     \Omega(n)
% \end{align*}
\end{lemma}

\begin{proof}
Consider the functions $\{ H_{\text{SCSC}, i}: \BR \times \BR \rightarrow \BR \}_{i=1}^n$ where
\begin{align*}
    H_{\text{SCSC}, i}(x, y) & = 
    \begin{cases}
    \frac{L}{2} \left( x^2 - y^2 \right) - n L R_x x,  &\text{ for } i = 1, \\
    \frac{L}{2} \left( x^2 - y^2 \right), &\text{ otherwise, }
    \end{cases}
\end{align*}
and $H_{\text{SCSC}} (x,y) = \frac{1}{n} \sum_{i=1}^n H_{\text{SCSC}, i} (x, y) = \frac{L}{2} (x^2 - y^2) - L R_x x$.
% Consider the minimax problem
% $$\min_{|x|\le R_x} \max_{|y| \le R_y} \tilde h(x, y).$$
It is easy to check that each component function $H_{\text{SCSC}, i}$ is $L$-smooth and $(\mu_x, \mu_y)$-convex-concave for any $0 \le \mu_x, \mu_y \le L$. 
Moreover, we have
\[
\max_{|y| \le R_y} H_{\text{SCSC}}(x,y) = \frac{L}{2} x^2 - L R_x x
\quad \text{and} \quad
\min_{|x| \le R_x} H_{\text{SCSC}}(x,y) = - \frac{L R_x^2}{2} - \frac{L}{2} y^2.
\]
% Then $\phi(x) = \max_{|y| \le R_y} = \frac{L}{2} x^2 - L R_x x$ and $\psi(y) = \min_{|x| \le R_x} = - \frac{L R_x^2}{2} - \frac{L}{2} y^2$.
Note that for $i \ge 2$, it holds that
\begin{align*}
    \nabla_x H_{\text{SCSC}, i}(x, y) = L x ~ \text{ and } ~
    \prox_{H_{\text{SCSC}, i}}^{\gamma}(x, y) = \left(\frac{x}{L\gamma + 1}, \frac{y}{L\gamma + 1}\right).
\end{align*}
This implies $x_t = x_0 = 0$ will hold till the PIFO algorithm $\fA$ draws $H_{\text{SCSC}, 1}$. 
Denote $T = \min\{t: i_t = 1\}$. 
Then, the random variable $T$ follows a geometric distribution with success probability $p_1$, and satisfies
\begin{align*}\label{eq:geo:one2}
    \pr{T \ge n/2} = (1 - p_1)^{\floor{(n-1)/2}} \ge (1 - 1/n)^{(n-1)/2} \ge 1/2,
\end{align*}
where the last inequality is according to that $h(\beta) = (\frac{\beta}{\beta + 1})^{\beta/2}$ is a decreasing function and $\lim_{\beta \to \infty} h(\beta) = 1/\sqrt{e} \ge 1/2$.
% By Equation (\ref{eq:geo:one2}), we have $ \pr{T \ge n/2} \ge 1/2.$
Consequently, for $N = n / 2$ and $t < N$, we know that
\begin{align*}
    &\quad \E\left( \max_{|y| \le R_y} H_{\text{SCSC}}(x_t, y) - \min_{|x| \le R_x} H_{\text{SCSC}}(x, y_t) \right) \\
    & \ge \E\left( \max_{|y| \le R_y} H_{\text{SCSC}}(x_t, y) - \min_{|x| \le R_x} H_{\text{SCSC}}(x, y_t) \bigg\vert t < T \right) \pr{T > t} \\
    &= \E\left( \max_{|y| \le R_y} H_{\text{SCSC}}(0, y) - \min_{|x| \le R_x} H_{\text{SCSC}}(0, y_t) \bigg\vert t < T \right) \pr{T > t}  \\
    & \ge \frac{L R_x^2}{2} \pr{T \ge N} \ge L R_x^2/4 \ge \eps.
\end{align*}
Therefore, in order to find $(\hat{x}, \hat{y}) \in \fX \times \fY$ such that 
\[
\E\left( \max_{|y| \le R_y} H_{\text{SCSC}}(\hat x, y) - \min_{|x| \le R_x} H_{\text{SCSC}}(x, \hat y) \right) < \eps, \]
PIFO algorithm $\fA$ needs at least $N = \Omega(n)$ queries.
\end{proof}

